Generalized Property-Directed Reachability for Hybrid Systems

Generalized property-directed reachability (GPDR) belongs to the family of the model-checking techniques called IC3/PDR. It has been successfully applied to software verification; for example, it is the core of Spacer, a state-of-the-art Horn-clause solver bundled with Z3. However, it has yet to be applied to hybrid systems, which involve a continuous evolution of values over time. As the first step towards GPDR- based model checking for hybrid systems, this paper formalizes HGPDR, an adaptation of GPDR to hybrid systems, and proves its soundness. We also implemented a semi-automated proof-of-concept verifier, which allows a user to provide hints to guide verification steps.

==> tmp <==
* The invariant checking performed in Algorithm 2 uses a sufficient condition. Why? The problem of continuous invariant checking was solved by Liu, Zhan & Zhao in EMSOFT'There. 11 is a *decision procedure* for invariant checking problems (if the ODEs are polynomial and all sets are semi-algebraic) which uses *necessary and sufficient conditions* and is fully automatic. I would strongly suggest the authors adopt it for this purpose. Another consequence of this decision procedure is fully automatic continuous invariant generation, which unfortunately is not practical using real quantifier elimination (but possible in principle); see https://dl.acm.org/citation.cfm?id=2038659  and their work with Kapur: http://lcs.ios.ac.cn/~znj/papers/festschrift-He.pdf

Minor comments:
 p.1 "IC3/PDR is initially proposed" -> "IC3/PDR was initially proposed"
 p.1 "it is then transferred" -> "it was then adapted"
 p.3 Definition 3.1 "where \sigma" - shouldn't this be \sigma_1 ?
 p.3. Definition 3.3 - What are the assumptions on the uniqueness and existence of solutions? What is the class of ODEs under consideration (linear/polynomial/elementary)? This is very important - please fix this.
 p.5. "Otherwise, the system is said to be unsafe" - this could be improved; right now it reads as though the system is unsafe if one cannot find an inductive invariant (even if there is one).
 p.7. "by Platzer et al. [30]" - [30] is a monograph by Platzer alone.
 p.12. "automated synthesizer of barrier certificates [31]" - this approach is not in practice fully automatic as it requires fixing a degree for a polynomial candidate. This whole passage strikes me as overly optimistic and unconvincing.

URL
